ChartX & ChartVLM: A Versatile Benchmark and Foundation Model for Complicated Chart Reasoning

Recently, many versatile Multi-modal Large Language Models (MLLMs) have emerged continuously. However, their capacity to query information depicted in visual charts and engage in reasoning based on the queried contents remains under-explored. In this paper, to comprehensively and rigorously benchmark the ability of the off-the-shelf MLLMs in the chart domain, we construct ChartX, a multi-modal evaluation set covering 18 chart types, 7 chart tasks, 22 disciplinary topics, and high-quality chart data. Besides, we develop ChartVLM to offer a new perspective on handling multi-modal tasks that strongly depend on interpretable patterns, such as reasoning tasks in the field of charts or geometric images. We evaluate the chart-related ability of mainstream MLLMs and our ChartVLM on the proposed ChartX evaluation set. Extensive experiments demonstrate that ChartVLM surpasses both versatile and chart-related large models, achieving results comparable to GPT-4V. We believe that our study can pave the way for further exploration in creating a more comprehensive chart evaluation set and developing more interpretable multi-modal models. Both ChartX and ChartVLM are available at: https://github.com/Alpha-Innovator/ChartVLM

==> tables/chartqa_test.tex <==


\begin{table}[t]
% \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    \small
	\centering	
    %\vspace{-3ex}
	\setlength{\tabcolsep}{1.1mm}{
    \begin{tabular}{c|c|ccc}
    
    \toprule
    \multirow{2}*{Model} &\multirow{2}*{Train Set }
    & \multicolumn{3}{c}{ChartQA Test}  \\    
    & & aug. \textcolor{blue!30}{\rule{0.7em}{0.55em}} & human \textcolor{red!30}{\rule{0.7em}{0.55em}} & avg. \\
    
    \midrule
     Deplot & ChartQA/PlotQA/C.D. & -  & - & -  \\   
    \bottomrule 
    
    \end{tabular}
    }
    \caption{\textbf{Evaluation on ChartQA test set using EM metric.}}

\label{tab:chartqa_test}
\end{table}

==> tables/chartqa_val.tex <==

\begin{table}[t]
% \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    \small
	\centering	
    %\vspace{-3ex}
	\setlength{\tabcolsep}{1.1mm}{
    \begin{tabular}{c|c|ccc}
    
    \toprule
    \multirow{2}*{Model} &\multirow{2}*{Train Set }
    & \multicolumn{3}{c}{ChartQA Val}  \\    
    & & aug. \textcolor{blue!30}{\rule{0.7em}{0.55em}} & human \textcolor{red!30}{\rule{0.7em}{0.55em}} & avg. \\
    
    \midrule
     VL-T5-OCR &ChartQA & - & - & 41.6  \\
     Tapas-OCR &ChartQA& - & - & 45.5 \\ 
     PaLI-17B &ChartQA& 64.9 & 30.4 & 47.6 \\ 
     Pix2Struct &ChartQA & 81.6 & 30.5 & 56.0  \\ 
     MatCha & ChartQA/PlotQA/C.D. & 90.2  & 38.2 & 64.2  \\
     Deplot & ChartQA/PlotQA/C.D. & 69.3  & 36.6 & 52.9  \\   
    \bottomrule 
    
    \end{tabular}
    }
    \caption{\textbf{Evaluation on ChartQA val set using EM metric.} Note that the ChartVLM model used for testing on ChartQA is same as that in Table~\ref{tab:compared_sota}}

\label{tab:chartqa_val}
\end{table}

==> tables/merge_effect.tex <==

\begin{table*}[!t]
    % \aboverulesep = 0.48mm
    % \belowrulesep = 0.48mm
    \small
	\centering	
 \setlength\tabcolsep{4pt}
    %  \vspace{-3ex}
	\resizebox{1\textwidth}{!}{
	\begin{tabular}	{l l |  c  c  c | c | c  c  c | c }
	\toprule	 	
	 \multirow{3}{*}{Model} & \multirow{3}{*}{\makecell[l]{\#Params}} &\multicolumn{4}{c|}{Tested on ChartQA val-set}   & \multicolumn{4}{c}{Tested on ChartX test-set}\\
	 & &    \multicolumn{3}{c}{Structural Extraction}& \multicolumn{1}{c|}{QA} & \multicolumn{3}{c}{Structural Extraction}  & \multicolumn{1}{c}{QA}  \\
	     
	& &  AP@Strict & AP@Slight & AP@High & GPT-score &  AP@Strict & AP@Slight & AP@High & GPT-score \\
	\midrule  
    \textit{~~Trained on ChartQA train set} \\
    \textbf{ChartVLM-B} & 8.3B 
    & 68.81 & 79.34 & 83.51 & 49.9
    & 1.48 & 2.22 & 3.78 & 24.4 \\
    
    \textbf{ChartVLM-L} & 14.3B
     & 69.55 & 78.44 & 83.65 & 58.8
    & 1.64 & 2.02 & 3.71 & 25.7 \\  

	\\	
	\midrule
	\multicolumn{2}{l}{\textit{~~Trained on merged set (ChartQA, PlotQA, Chart2Text, SimChart9K)}} \\ 
    \textbf{ChartVLM-B} & 8.3B 
    & 70.91 & 82.81 & 85.72 & 54.2 
    &18.49 & 25.11 & 30.26 & 36.5 \\
    
    \textbf{ChartVLM-L} & 14.3B
     & \textbf{73.27} & \textbf{83.68} & \textbf{86.21} & 59.3 
    & \textbf{23.16} & \textbf{29.50} & \textbf{35.26} &  40.7 \\  
    \bottomrule
	\end{tabular}
	}
    \vspace{-10pt}
	\caption
	{
	\small	
        The effectiveness of the proposed ChartX, where we employ two training settings: a) training using only ChartQA train set, and b) training using the merged set of ChartQA, PlotQA, Chart2Text, SimChart9K.
	}
	\label{tab:chartx_effect}
 \vspace{-1ex}
\end{table*}

==> tables/related_charts.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{1.0}{
\begin{tabular}{lcccccc@{}}
\toprule
\multirow{2}{*}{Datasets}           & \multirow{1}{*}{\# Chart}            & \# Chart & \# Task & \# Evaluation & \# Evaluation Instruction-& Open- \\ 
  & Topic & Type & Type & Chart Images & following Data & source\\ 
\midrule
\textit{~~Single-task Benchmarks} \\
PlotQA \citep{methani2020plotqa}          & N/A               & 3   & 1                  & 33.7K           & 4.3M                         & \Checkmark                 \\
Chart-to-text \citep{obeid2020chart}        & 6          & 6       & 1         & 6.6K            & 6.6K                              & \Checkmark                 \\
ChartQA \citep{masry2022chartqa}   & 15   & 3         & 1    & 1.6K                & 2.5K                         &  \Checkmark               \\
OpenCQA  \citep{kantharaj2022opencqa}    & 10                     & 5     & 1             & 1.2K & 1.2K                      & \Checkmark                    \\ 
\midrule
\textit{~~Multi-task Benchmarks} \\
ChartLlama \citep{han2023chartllama}        & N/A              & 10      & 7          & 0.5K            & N/A                          & \Checkmark\textsuperscript{\kern-0.89em\tiny\XSolidBrush}             \\
ChartBench  \citep{xu2023chartbench}      & N/A             & 9       & 4          & 2K             & 16K                             & \XSolidBrush                 \\
MMC \citep{liu2023mmc}          & 5                    & 6         & 9        & 2.1K        & 2.1K                & \XSolidBrush               \\
ChartX     & 22   & 18 & 7 & 6K & 48K & \Checkmark  \\
\bottomrule
\end{tabular}}
\caption{Comparison with existing chart-related benchmarks.}
\end{table*}

==> tables/related_charts_2.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{1.0}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
Evaluation Set                      & \# Chart type & \# Visual Chart  & \# Language Chart & \# Task type & Open-source & \# Topic \\ 
\midrule
\multicolumn{1}{c}{ChartQA~\citep{masry2022chartqa}} & 3            & 1K          & 1.9K                     & 1           & T            & 4       \\
\multicolumn{1}{c}{MMC~\citep{liu2023mmc}} & 6            & 0.8K          & 1.9K                     & 9           & T            & -       \\
ChartX (ours)      & 18 & 6K & 48K & 7 & T & 22 \\
\bottomrule
\end{tabular}}
\end{table*}
